Pressure jump interface law for the Stokes-Darcy coupling: Confirmation by direct numerical simulations

It is generally accepted that the effective velocity of a viscous flow over a porous bed satisfies the Beavers-Joseph slip law. To the contrary, interface law for the effective stress has been a subject of controversy. Recently, a pressure jump interface law has been rigorously derived by Marciniak-Czochra and Mikeli\'c. In this paper, we provide a confirmation of the analytical result using direct numerical simulation of the flow at the microscopic level.

==> test <==
%
\input{numerical_setting_introduction} 

\subsection{Finite Element Formulation of the Microscopic Problem}
\label{Numset}
To numerically solve the problems we consider the finite element method and we give exemplary in this subsection the formulation of the microscopic problem \eqref{1.3}-\eqref{1.5}. For a more thorough introduction into the theory of finite elements, we refer to standard literature such as \cite{Ciarlet:2002} or \cite{BrennS:2002}.

The natural setting of the finite element approximation of the problem is its weak formulation, shown below.
We first introduce the spaces
\begin{align}
V(\Oe) &:= \Set{\mathbf{v} \in H^1(\Oe)^2\ \big|\ \mathbf{v}  =0 \; \hbox{on } \ \p \Omega \setminus \Gammaper, \mathbf{v} \hbox{ is } L\text{-periodic in } x_1},\\
L_0(\Oe) &:= \Set{ p \in L^2(\Oe)\ \big | \ \int_{\Oe} p \ dx = 0},
\end{align}
%
where $L^2(\Oe)$ is the space of square-integrable functions in $\Oe$, i.e. $\displaystyle \int_{\Oe} \abs{u(x)}^2\,dx < \infty$, and $H^1(\Oe)$ is the space of square-integrable functions, with first derivatives also square-integrable.
%
 
The weak formulation of problem \eqref{1.3}-\eqref{1.5} reads as follows:
%
\begin{problem}[Microscopic Problem in Weak Formulation]\label{prob.micro_weak}
Find a pair $(\ve,p^\ep) \in V(\Omega^\epsilon)\times L_0(\Oe)$, such that
\begin{align}
\int_{\Oe} \nab \ve \cdot \nab \vphi \ dx + \int_{\Oe} p^\ep \nab \cdot \vphi \ dx &= \int_{\Oe} \mathbf{e}_1 \cdot \vphi \ dx &&\forall \vphi \in V(\Oe),\\
\int_{\Oe} \nab \cdot \ve \ \psi \ dx &= 0 &&\forall \psi \in L_0(\Oe).
\end{align}
\end{problem}

We use finite elements to discretize this problem and consider a decomposition $\grid$ of the domain into so called cells, whose union constitutes an approximation of the problem geometry, i.e. $\grid = \Set{\cell}$. 
We consider grids made of convex quadrilateral, whose aspect ratio are bounded. This property is called shape regularity. 
The cells are constructed via a set of polynomial transformations $\Set{\transf_\cell}_{\cell \in \grid}$ of a unit reference cell $\hat \cell$, see also Remark~\ref{rem.transformation}. The diameters $h_\cell$ of the cells define a mesh parameter $h$ by the piecewise constant function $h_{|\cell} = h_\cell$. 
On the grid we define for $s \in \mathbb N$
%the  space $V_h \subset V$ as 
the finite dimensional space 
%of polynomial functions
% \begin{align}
% V_h := \{v_h ~|~ {v_h}_{|K} \in Q^s(K), K \in \grid \},
% \end{align}
\begin{align}
\mathcal{S}_h^s(\Oe):=\Set{v_h\in C^0(\overline {\Oe})\ \big| \ {v_h}_{|\cell} \in Q^s(\cell), \cell \in \grid },
\end{align}
where $C^0(\overline \Oe)$ is the space of continuous functions on $\overline {\Oe}$. Let $P^s(\hat \cell)$ be space of polynomials of order lower or equal to $s$, then the space 
\begin{align}
Q^s(\cell)= \Set{p: T \to \mathbb{R}\ |\ p\left(\transf_\cell(\cdot)\right) \in  P^s(\hat \cell)}
\end{align}is the space of functions obtained by a transformation of bilinear ($s=1$), biquadratic ($s=2$) and in general higher order polynomials defined on the unit reference cell $\hat \cell$. 
%

For convergence results we consider a family of grids obtained by either uniform or local refinement of an initial regular grid.

\begin{remark}[Boundary Approximation]\label{rem.transformation}
Since the considered domains have curved boundaries we correspondingly use cells with curved boundaries (i.e. isoparametric finite elements) to get a better approximation. 
Condidering the space $\mathcal{S}_h^2$ for the velocity we use biquadratic transformations of the unit cell $\hat \cell$.
\end{remark}
%
For the discretization of the Stokes system we use the Taylor-Hood elements that use the ansatz space $V_h(\Oe):=\left(\mathcal{S}^2_h(\Oe)\right)^2 \cap V(\Oe)$ for the velocity and $L_h(\Oe):=\mathcal{S}_h^1(\Oe)$ for the pressure.
This discretization is inf-sup stable (cf. \cite{BrezzF:1991}), so we do not need stabilization terms to solve the saddle point corresponding to the Stokes system, as for example in \cite{JaegerMN:2001}.

The \textbf{finite element approximation} of the microscopic problem is obtained by replacing the (infinite dimensional) function spaces $V(\Oe)$ and $L_0(\Oe)$ by their discretized counterparts $V_h(\Oe)$ resp. $L_h(\Oe)$.
\begin{problem}[Finite Element Approximation of Microcopic Problem]\label{prob.micro_fe}
Find a pair $(\veh,p^\ep_h) \in V_h(\Omega^\epsilon)\times L_h(\Oe)$, such that
\begin{align}
\int_{\Oe} \nab \veh \cdot \nab \vphih \ dx + \int_{\Oe} p^\ep_h \nab \cdot \vphih \ dx &= \int_{\Oe} \mathbf{f} \cdot \vphih \ dx &&\forall \vphih \in V(\Oe),\\
\int_{\Oe} \nab \cdot \veh \ \psi_h \ dx &= 0 &&\forall \psi_h \in L_0(\Oe)
\end{align}
and $\int_{\Oe} p^\ep_h\ dx = 0$.
\end{problem}

As shown in Section~\ref{problem_setting}, see also \cite{JaegerM:1996,JaegerM:2000,JaegerM:2009},  the Navier boundary layer problem (\ref{BJ4.2})-(\ref{4.6}) has to be solved to determine the constants \cbl{} and \cblw{} in the interface law \eqref{4.95} and the first of \eqref{Presspm2A}.
Next subsection is thus dedicated to the numerical determination of these constants and we will show in sections \ref{sec:case_I} and  \ref{sec:case_II} by direct numerical solving of the microscopic problem that the constant $\cblw$ is related to the pressure difference between the free fluid and the porous part.

As previously explained we use two different kinds of inclusion in the porous part, \textbf{circles} and \textbf{ellipses}. 
The geometries of the unit cells $Y = (0.1)^2$, see Figure~\ref{fig.inclusions}, for these two cases are as follows:
\begin{enumerate}
\item the solid part of the cell $Y_s$ is formed by a circle with radius $0.25$ and center $(0.5, 0.5)$.
\item $Y_s$ consists of an ellipse with center $(0.5, 0.5)$ and semi-axes $a=0.357142857$ and $b=0.192307692$, which are rotated anti-clockwise by $45^\circ$. 
\end{enumerate}
\begin{figure}[hbt]
\centering
 \begin{subfigure}[htb]{0.3\textwidth}
\centering 
\includegraphics[trim=54mm 80mm 21mm 83mm, clip, width =0.8\textwidth]{../Figures/mesh_circle.pdf}
\caption{Circle}\label{subfig.circle}
\end{subfigure}
\begin{subfigure}[htb]{0.3\textwidth}
\centering 
\includegraphics[trim=54mm 80mm 21mm 83mm, clip,width=0.8\textwidth]{../Figures/mesh_ellipse.pdf}\caption{Ellipse}\label{subfig.ellipse}
\end{subfigure}
\caption{Mesh of the fluid part of the unit cell for the two types of inclusions: circles (\subref{subfig.circle}) and ellipses (\subref{subfig.ellipse}).}\label{fig.inclusions}
\end{figure}
The circle geometry is a case of axis symmetric geometry with respect to the axis $y$, perpendicular to the interface $\Sigma$, for which we expect from the theory that is $\cblw=0$.

All computations are done using the toolkit \texttt{DOpElib} (\cite{GollWW:2012}) based upon the C++-library \texttt{deal.II} (\cite{BangeHK:2007}).
%All computations were done using the C++-library deal.II (\cite{BangeHK:2007}).
%\todo{Reference \texttt{DOpElib}}

%\subsection{Navier boundary problem and determination of slip velocity and pressure jump conditions}
\subsection{Finite element formulation of the Navier boundary layer problem}
\label{sec:Navier boundary problem}
%
The Navier boundary layer problem (\ref{BJ4.2})-(\ref{4.6}) is defined on $\Zbl:=Z^+ \cup \IF \cup Z^-$, where $\Gamma=(0,1)\times\{0\}$, $Z^+=(0,1)\times(0,+\infty)$ and $Z^-=\cup_{k=1}^\infty(Y_f - \{0,k\})$, with $Y_f$ the fluid part of the pore, see Figure~\ref{fig.boundary_layer_domain}.

After \cite{JaegerM:1996} and \cite{JaegerMN:2001}, it is known that $\boldsymbol\betabl$ converges exponentially towards $(\cbl,0)$ and $\wbl$ towards $\cblw$ in $Z^+$ for increasing $y_2$. On the porous side it has been also shown in the same references that the pressure $\wbl$ and the velocity $\betabl$ converge exponentially towards zero. In addition it has been shown therein that
\begin{subequations}\label{cbl_cblw}
\begin{align}
\cbl &= \int_0^1 \betabl_{1}(y_1,0) \ dy_1,\\
\cblw &= \int_0^1 \wbl(y_1,0) \ dy_1, = \int_0^1 \wbl(y_1,1) \ dy_1
\end{align}
\end{subequations}
where $(\betabl, \wbl)$ ist the solution of (\ref{BJ4.2})-(\ref{4.6}). Both this integrals are well defined since $\betabl$ and $\wbl$ are smooth in $Z^+$ up to the interface $\Sigma$.

Since we can not deal with infinitely large domains, we consider a cut-off domain for numerical calculations defining the finite slab $\Zkl:=\Zbl\cap (0,1)\times(-l,k)$, $ k, l>0$. The distance of the cut-off from the interface, determined by $k$ and $l$, has to be taken large enough considering the exponential decay to reduce the approximation error introduced by cutting the domain. 

At the newly introduced parts of the boundary, namely $\Gamma_{ k} = (0,1)\times \{k\}$ and $\Gamma_{ l} = (0,1)\times \{-l\}$, we have to set some appropriate boundary conditions. We follow \cite{JaegerMN:2001} and put zero Dirichlet condition for the two velocity components on $\Gamma_l$, while on $\Gamma_k$ a zero Dirichlet condition for the vertical component as well as zero normal flux of the first velocity component is imposed.

% In view of this, we consider a cut-off domain for numerical calculations defining the finite slabs $Z^+_k:=(0,1)\times(0,k)$, $Z^-_l=\cup_{n=1}^l \left( Y_f - \{0,n\} \right)$, $ k, l>0$. At the newly introduced parts of the boundary, namely $\Gamma_{\rm k} = (0,1)\times \{k\}$ and $\Gamma_{\rm l} = (0,1)\times \{-l\}$, we have to set some appropriate boundary conditions. We impose $

In the following we give the finite element approximation of the cut-off Navier Boundary Layer problem:
\begin{problem}[Cut-off Navier Boundary Layer]\label{prob.bl}
Find $\boldsymbol\beta^{bl}_h \in \tilde V_h(\Zkl)$ and $\omega^{bl}_h \in L_h(\Zkl)$, such  that 
\begin{align}
\int_{\Zbl} \nabla \boldsymbol\beta^{bl}_h \cdot \nabla \boldsymbol\varphi + \omega^{bl}_h \ \nabla \cdot \boldsymbol\varphi\ dx&= -\int_{\IF}\varphi_1\ dx, && \forall \boldsymbol\varphi \in\tilde V_h(\Zkl),\\
 \int_{\Zbl} \nabla \cdot \boldsymbol\beta^{bl}_h \ \psi\ dx&= 0,  && \forall \psi \in L_h(\Zkl),%\\
\end{align}
\end{problem}
where the space for the velocity incorporates the Dirichlet boundary conditions on $\Gamma_k$ and $\Gamma_l$ and is thus defined as follows
%
\begin{align}
\tilde V_h(\Zbl) := \{\mathbf{v}_h \in C^0(\Zbl)~|~& {\mathbf v_h}_{|K} \in Q^2(K),K \in {\cal T}_h,\notag \\
&\mathbf v_h = 0 {\rm ~on} \cup_{n=1}^l (\partial Y_s - (0,n)),\notag \\
&\mathbf v_h = (0,0) \text{ on } \Gamma_l \text{ and } v_{h,1} =0 \text{ on } \Gamma_k,\notag\\
&\mathbf v_h {\rm ~is~} y_1-\mbox{periodic with period } 1 \}, \label{Space1}
\end{align}
%
with  $\partial Y_s$ the boundary of the inclusions in the pore domain, as shown in Figure~\ref{?}. \todo{Picture of unit cell}

With the numerical solution of Problem~\ref{prob.bl} we approximate the constants \cbl{} and \cblw{} for the considered inclusions. The approximations $\cblh$ and $\cblwh$ are then calculated by replacing in \eqref{cbl_cblw} the functions $(\betabl, \wbl)$ with their discretized counterparts, the index $h$ indicates the approximation due to discretization. As a remark, we have observed that to enhance the numerical approximation the use of the second formulation of \cblw{}, i.e. the integral of the pressure along the line $\Set{y\in \Zbl\ | \ y_2=1}$, has to be preferred. 

A very accurate approximation of \cblw{} is needed to show in Section~\ref{numerical_confirmation} convergence results for $\epsilon \rightarrow 0$.
The approximation of the cut-off problem by finite elements introduces two different sources of error: \textbf{cut-off error} and \textbf{discretization error}. In our computations, we set $k=l$ and compute the solution of Problem~\ref{prob.bl} for $1\leq k \leq 5$ on a family of hierarchic adaptively refined meshes.
To obtain convergence results in Section~\ref{numerical_confirmation}, it is important to control the cut-off and discretization errors and balance them to reduce the computational costs.
To balance the two errors we should cut the domain so that the order of the cut-off error equals that of the discretization error. To this aim we need to control the discretization error by a reliable estimation. Since we are interested on the calculation of \cbl{} and \cblw{}, we want to control directly the errors $J_1=|\cbl{} - \cblh|$ and $J_\omega=|\cblw{} - \cblwh|$. Using a local refinement strategy we obtain grids that are not quasi-uniform, i.e. the following condition is not always fulfilled:
\begin{align}
h_{max}^i \leq C h_T \quad \forall T \in \gridi,
\end{align}
where $\gridi$ is the $i^{th}$ grid of the family obtained by subsequent refinement and $h_{max}^i$ is the maximal cell diameter of grid $i$.
As a consequence, we can not expect to estimate the errors $J_1$ and $J_\omega$ comparing two successive grids. We adopt instead the Dual Weighted Residual (DWR) method from \cite{BeckeR:2001} that gives an a posteriori estimation of the discretization error with respect to a given functional exploiting the solution of a proper adjoint equation.

We use local error indicators derived by the DWR method to control the local mesh refinement. 
The triangulation is adaptively refined until the estimated discretization error is smaller than a given tolerance. 
The reliability of this estimator, in this context, is yet justified by the fact that it estimates the exact order of the discretization error as shown below.
We have performed an additional check to assure that the order of the error is indeed the one estimated.
Since to check the convergence we do not have the exact solution, but we can rely on the best approximation property of Galerkin approximations on quasi-uniform meshes, we perform the following verification. 

We consider the solution on the finest local refined mesh as a reference solution and check if solutions on a family of uniformly refined meshes converge towards that reference value.
We use this series of grids to check the reliability of the error estimator. To this end we evaluate the error estimator $\eta$ on family of uniformly refined grids and compare this value using the reference solution computed on much finer local refined mesh, i.e. $C_{1,h}^{bl,ref} - C_{1,h}^{bl,unif}$ and $C_{\omega,h}^{bl,ref} -  C_{\omega,h}^{bl,unif}$, where $C_{1,h}^{bl,ref}$ resp. $C_{\omega,h}^{bl,ref}$ is calculated on local refined meshes while $C_{1,h}^{bl,unif}$ resp. $C_{\omega,h}^{bl,unif}$ on uniformly refined meshes. After this verification, we conclude that the DWR based estimator is reliable, since (cf. Table~\ref{tab.results_global_mesh_refinement}) the solution on uniform meshes converges towards our reference solution and the error estimator is of the same order as the one given by the reference value. We have used grids with up to around 3.9 millions of degrees of freedom for the verification with uniformly refined meshes obtaining an error estimation of order $\eta(\cbl) \sim 10^{-10}$ and $\eta(\cblw) \sim 10^{-9}$. 
Table~\ref{tab.results_global_mesh_refinement} shows the efficiency of the error estimator, i.e. 
%
\begin{align*}
I_{eff}(\cbl) = \frac{C_{1,h}^{bl,ref} - C_{1,h}^{bl,unif}}{\eta(\cbl)}, \quad I_{eff}(\cblw) = \frac{C_{\omega,h}^{bl,ref} - C_{\omega,h}^{bl,unif}}{\eta(\cbl)},
\end{align*}
from which the reliability of the error estimation can be deduced.

As tolerance for calculations of the two constants to be used in Section~\ref{numerical_confirmation} we have adopt the condition $\eta(\cbl)$, $\eta(\cblw) < 10^{-11}$, where $\eta(\cbl)$ and $\eta(\cblw)$ are DWR error estimators respectively of $|\cbl - C_{1,h}^{bl}|$ and $|\cblw - C_{\omega,h}^{bl}|$ using local refined meshes with up to 7 millions of degrees of freedom.

In \cite{JaegerMN:2001} it is shown that the cut-off error decays exponentially with $k$ and $l$. 
To find the optimal cut-off level $l, k$ we perform a convergence check taking as reference value the constants computed on $Z_5^5$, i.e. $\cblh(Z_5^5)$ resp. $\cblwh(Z_5^5)$.
Figure~\ref{fig.exp_convergence} shows the error between the constants computed on $\Zkl$ with $k=l =1,\dots, 4$ and the reference values on $Z_5^5$. 
The exponential decay of the cut-off error with the distance from interface can be observed for both approximations. Furthermore, it can be observed that the error $|\cblh(Z_k^l) - \cblh(Z_5^5)|$ is of the order of the discretization error, i.e. $10^{-12}$, for $k,l\geq3$ for \cbl and $k,l\geq 4$ for \cblw.

In the following, we use approximations computed with local mesh refinement and $k,l=5$ maintaining the simplified notation \cblh{} and \cblwh{}.
For details on the used local refinement strategy see \cite{Richter:Diss}.

The calculated constants and the respective error estimation are listed in Table~\ref{tab.results_c1_cw}.

%
\begin{figure}[hbt]
\centering
\resizebox{0.5\textwidth}{!}{\input{../Figures/exp_convergence.tex}}
\caption{Difference between the computed constants on domains with increasing length and $\cblh(Z_5^5)$ resp. $\cblwh(Z_5^5)$.}\label{fig.exp_convergence}
\end{figure}
%

\begin{table}
\centering 
\begin{tabular}{r|ccc|ccc}
\toprule
\# DoFs & $C_{1,h}^{bl,ref} - C_{1,h}^{bl,unif}$& $\eta_{\cbl}$ & $I_{eff}(\cbl)$& $C_{\omega,h}^{bl,ref} -  C_{\omega,h}^{bl,unif}$& $\eta_{\cblw}$ & $I_{eff}(\cblw)$\\
\cmidrule(lr){1-7}
	   1\,096 & -4.52E-04 & -2.54E-03 & 5.61 & 2.99E-02   &	-9.03E-03&	-0.30 \\
	   4\,142 & -7.49E-05 & -2.75E-04 & 3.67 & -2.07E-04  &  -1.02E-03 &	4.92  \\
	  16\,066 & -1.10E-05 & -1.87E-05 & 1.71 & 3.66E-06   &  -9.70E-05 &	-26.50\\
	  63\,242 & -9.60E-07 & -1.11E-06 & 1.15 & -9.72E-07  &  -4.78E-06 &	4.92  \\
	 250\,906 & -6.83E-08 & -7.60E-08 & 1.11 & -9.67E-08  &  -3.15E-07 &	3.26  \\
	 999\,482 & -4.54E-09 & -5.36E-09 & 1.18 & -9.03E-09  &  -2.77E-08 &	3.07  \\
	3\,989\,626 & -2.90E-10 & -3.82E-10 & 1.32 & -1.28E-09  &  -3.67E-09 &	2.85  \\
\bottomrule 
\end{tabular}
\caption{Results of the approximation of the constants \cbl{} and \cblw{} by uniform mesh refinement. }\label{tab.results_global_mesh_refinement}
\end{table}
%
\begin{table}
\centering 
\begin{tabular}{c|cccc}
\toprule
k,l&\cblh& $\eta(\cbl{})$ &\cblwh&$\eta(\cblw{})$\\
\cmidrule(lr){1-5}
&\multicolumn{4}{c}{circular inclusions}\\
\cmidrule(lr){2-5}
1  &-0.3038181652339	&	1.9E-12	&	-&-\\
2  &-0.3038219423526	&	2.0E-12	&	-&-\\
3  &-0.3038219423790	&	2.0E-12	&	-&-\\
4  &-0.3038219423789	&	2.0E-12	&	-&-\\
5  &-0.3038219423786	&	??E-12 	&	-&-\\
\midrule
	&\multicolumn{4}{c}{oval inclusions}\\
\cmidrule(lr){2-5}
1  & -0.2694539064491   & 4.3E-12	   &	-0.2413211012145	& 2.1E-11\\
2  & -0.2694545953967	& 1.4E-12      &	-0.2409146886571	& 7.3E-12\\
3  & -0.2694545953993	& 3.1E-12      &	-0.2409148310717	& 7.2E-12\\
4  & -0.2694545953993	& 2.1E-12      &	-0.2409148310975	& 8.5E-12\\
5  & -0.2694545953985	& 2.0E-12      &	-0.2409148310959	& 8.6E-12 \\ 		
\bottomrule 
\end{tabular}
\caption{Results of the approximation of the constants \cbl{} and \cblw{} as well as the estimated discretization error $\eta$ for different domain-lengths. }\label{tab.results_c1_cw}
\end{table}
%

\subsection{Cell problem and determination of the permeability}
To confirm

Next we present the permeabilities $K$ in the case of circular and oval inclusions. To compute these, we first have to solve additional cell problems.
To give the weak form of these problems, we need the following function space
\begin{align}
\hat V(Y_f) &:= \Set{\mathbf{v} \in H^1(Y_f)^2\ | \ \mathbf{v}  =0 \; \hbox{on } \ \p Y_s, \mathbf{v} \hbox{ is } 1\text{-periodic}}.
\end{align}

Following the derivation of Darcy's Law by homogenization, the matrix $K$ is defined as
\begin{align}
K_{ij} = \int_{Y_f} w_j^i\ dy,\quad 1\leq i,j\leq2,
\end{align}
where $\mathbf w$ is a part of the solution of the following \textbf{cell problem}.
\begin{problem}[Cell Problem]\label{prob.cell_problem}
Let $1\leq i,j\leq2$. Find a velocity field $\mathbf w^i \in \hat V(Y_f)^2$ and a pressure $\pi^i \in L_0(Y_f)$, such that,
\begin{align}
\int_{Y_f} \nabla \mathbf w^{i} \cdot \nabla \boldsymbol\varphi + \pi^{i} \ \nabla \cdot \boldsymbol\varphi\ dx&= \int_{Y_f}\varphi_i\ dx, && \forall \boldsymbol\varphi \in \hat V(Y_f),\\
 \int_{Y_f} \nabla \cdot \mathbf w^i \ \psi\ dx&= 0,  && \forall \psi \in L_0(\Zbl).%\\
\end{align}
\end{problem}

We do not state the finite element formulation of the cell problem as one has only to switch ansatz- and test spaces in Problem~\ref{prob.cell_problem} as it was shown in the previous sections. We use again the Tayler-Hood element in combination with an adaptive algorithm based on the DWR method to compute the reference-values for the permeability matrix $K$.

The computed reference values for further use are
\begin{align}  K^{circ}_h &= k^{circ}_h Id \approx {0.01990143534975}Id
\end{align}
with an estimated discretization error of $1.38\cdot 10^{-11}$. For the case with an ellipse as inclusion, we use the value
\begin{align}
K^{oval}_h &= \left(
\begin{array}{cc}
K_{h,11} & K_{h,12} \\
K_{h,12} & K_{h,22} \\
\end{array}
\right) \approx \left(
\begin{array}{cc}
0.0159787174788 &  0.00303449804138  \\
0.00303449804138 & 0.0159787174788
\end{array}\right)                             .
\end{align}
with an discretization error of $2.76\cdot10^{-12}$ for  $K_{h,11}$ and  $1.10\cdot10^{-13}$ for  $K_{h,12}$.
\begin{itemize}
\item \todo{pictures of the solution?}
\end{itemize}


